Findings of the The RuATD Shared Task 2022 on Artificial Text Detection in Russian

We present the shared task on artificial text detection in Russian, which is organized as a part of the Dialogue Evaluation initiative, held in 2022. The shared task dataset includes texts from 14 text generators, i.e., one human writer and 13 text generative models fine-tuned for one or more of the following generation tasks: machine translation, paraphrase generation, text summarization, text simplification. We also consider back-translation and zero-shot generation approaches. The human-written texts are collected from publicly available resources across multiple domains. The shared task consists of two sub-tasks: (i) to determine if a given text is automatically generated or written by a human; (ii) to identify the author of a given text. The first task is framed as a binary classification problem. The second task is a multi-class classification problem. We provide count-based and BERT-based baselines, along with the human evaluation on the first sub-task. A total of 30 and 8 systems have been submitted to the binary and multi-class sub-tasks, correspondingly. Most teams outperform the baselines by a wide margin. We publicly release our codebase, human evaluation results, and other materials in our GitHub repository (https://github.com/dialogue-evaluation/RuATD).

==> tables/corpus_table/corpus_table.tex <==
\begin{table*}[t!] % [H]
    \centering
    \begin{tabular}{c|c|c|l}
        \toprule

        \textbf{Task} & \textbf{Text Generator} & \textbf{Domain} & \textbf{Num. samples} \\
        \midrule
        \textbf{Machine Translation} &
            \begin{tabular}{@{}c@{}c@{}c@{}}
                Human \\ OPUS-MT \\ M-BART50 \\ M2M-100
            \end{tabular} &
            
            \begin{tabular}{@{}c@{}}
                Tatoeba \\ WikiMatrix  \\
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                35860
            \end{tabular}
        \\\midrule
        
        \textbf{Back Translation} &
            \begin{tabular}{@{}c@{}c@{}c@{}}
                Human \\ OPUS-MT \\ M-BART50 \\ M2M-100 
            \end{tabular} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
                Strategic documents \\ News \\ Prozhito \\ RNC \\ Wikipedia \\ Tatoeba \\ WikiMatrix 
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                35588
            \end{tabular}
        
        \\\midrule
        
        \textbf{Paraphrase Generation} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
                Human \\ mT5-Small \\ mT5-Large \\ ruT5-Base-Multitask \\ ruGPT2-Large \\
                ruGPT3-Large
            \end{tabular} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
                Strategic documents \\ News \\ Prozhito \\ RNC \\ Wikipedia \\ Social media 
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                44298
            \end{tabular}
        
        \\\midrule
        
        \textbf{Simplification} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
                Human \\ mT5-Large \\ ruT5-Large \\ ruGPT3-Small \\ ruGPT3-Medium \\ ruGPT3-Large
            \end{tabular} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
            Strategic documents \\ News \\ Prozhito \\ RNC \\ Wikipedia \\ Social media 
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                44700
            \end{tabular}
        
        \\\midrule
        
        \textbf{Summarization} &
            \begin{tabular}{@{}c@{}c@{}}
                Human \\ M-BART \\ ruT5-Base
            \end{tabular} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}}
            Strategic documents \\ News \\ Prozhito \\ RNC \\ Wikipedia 
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                17164
            \end{tabular}
        
        \\\midrule
        
        \textbf{Zero-shot Generation} &
            \begin{tabular}{@{}c@{}c@{}c@{}}
                Human \\ ruGPT3-Small \\ ruGPT3-Medium \\ ruGPT3-Large
            \end{tabular} &
            \begin{tabular}{@{}c@{}c@{}c@{}c@{}}
            Strategic documents \\ News \\ Prozhito \\ RNC \\ Wikipedia 
            \end{tabular} &
            
            \begin{tabular}{@{}c }
                37499
            \end{tabular}
        
        \\\midrule
    

    \end{tabular}
    \caption{Text generators, domains and the final number of samples per task}
    \label{tab:tgms}
\end{table*}


==> tables/leaderboards/leaderboards.tex <==
\begin{table}
\centering
\begin{tabular}{lr | lr}
\toprule
\multicolumn{2}{c|}{Binary sub-task}  & \multicolumn{2}{c}{Multi-class sub-task} \\
Team &    Accuracy & Team & Accuracy \\
\midrule
MSU &  0.82995 & Posokhov Pavel &  0.65035\\
Igor &  0.82725 & Yixuan Weng &  0.64731 \\
Orzhan &  0.82629 & Orzhan &  0.64573 \\
mariananieva &  0.82427 & MSU &  0.62856\\ 
Ivan Zakharov &  0.82294 & \cellcolor[gray]{0.8}BERT baseline  &   \cellcolor[gray]{0.8} 0.59813\\ 
Yixuan Weng &  0.81767 & Nikita Selin &  0.58967\\
ilya koziev &  0.81699 & Victor Krasilnikov &  0.55012\\
miso soup &  0.81178 & Petr Grigoriev &  0.45814\\
Eduard Belov &  0.80862 &\cellcolor[gray]{0.8}TF-IDF baseline &  \cellcolor[gray]{0.8}0.44280\\
Posokhov Pavel \checkmark &  0.80630 & Anastasiya Shabaeva &  0.05411\\ Kirill Apanasovich &  0.80308 \\
Tumanov Alexander &  0.79778 \\ 
\cellcolor[gray]{0.8}BERT baseline &  \cellcolor[gray]{0.8} 0.79666 \\ 
     Elizaveta Nosova &  0.79595 \\
              mipatov &  0.78591 \\
               akstar &  0.78442 \\
         Nikita Selin &  0.78228 \\
        David Avagyan &  0.77869 \\
      Mikhail Yumanov &  0.77181 \\
    Gregory Kuznetsov &  0.75237 \\
   Anastasiya Shabaeva &  0.75178 \\
           Shershunya &  0.74534 \\
 Ekaterina Kostrykina &  0.74326 \\
   Victor Krasilnikov &  0.74091 \\
                Alena &  0.73589 \\
 Alexander Tesemnikov &  0.73204 \\
           Lera Lelik &  0.72727 \\
    Dmitriy Vahrushev &  0.71559 \\
      Molostvov Pavel &  0.68543 \\
           Mental Sky &  0.65326 \\
       Petr Grigoriev &  0.64232 \\ 
      \cellcolor[gray]{0.8}TF-IDF baseline  &  \cellcolor[gray]{0.8} 0.64223 \\
\bottomrule
\end{tabular}
\caption{Left: binary leaderboard; right: multi-class leaderboard. Baseline submissions are colored in grey}
\label{tab:leaderboards}
\end{table}



==> tables/metrics_minipage.tex <==
\begin{table}[!htb]
\centering
\makebox[0pt][c]{\parbox{1.0\textwidth}{%
    \raisebox{0ex}{
        \begin{minipage}[c]{0.49\hsize}\centering
            \begin{tabular}{ll|c|c}
            \toprule
             &   & \textbf{H} & \textbf{M} \\
             & \textbf{k} &           &            \\
            \midrule
            & \textit{1} &  0.35 &   0.40 \\
            \textbf{Dist-k} & \textit{2} &  0.75 &   0.76 \\
                 & \textit{4} &  0.74 &   0.77 \\
            \midrule
            & \textit{1} &  7.86 &   7.30 \\
            \textbf{Ent-k} & \textit{2} &  9.99 &   9.03\\
                 & \textit{4} &  10.16 &   9.19 \\
            \bottomrule
            \end{tabular}
        \end{minipage}
    }
    \hfill
    \raisebox{0.35ex}{
        \begin{minipage}[c]{0.49\hsize}\centering
            \begin{tabular}{l|c|c}
            \toprule
             &       \textbf{IPM} &  \textbf{Num tokens} \\
             &           &             \\
            \midrule
            \textbf{Back Translation} & 0.88 & 12.9 \\
            \textbf{Machine Translation} & 0.89 & 11.5 \\
            \textbf{Zero-shot Generation} & 0.85 & 141.5 \\
            \textbf{Paraphrase Generation} & 0.85 & 13.0 \\
            \textbf{Simplification} & 0.86 & 18.3 \\
            \textbf{Summarization} & 0.86 & 33.5  \\
            \bottomrule
            \end{tabular}
        \end{minipage}
    }
    
    \begin{minipage}[t]{0.49\textwidth}
        \caption{Dist-\textit{k} and Ent-\textit{k} metrics for diversity.}
        \label{tab:dist-ent}
    \end{minipage}%%%
    \hfill
    \begin{minipage}[t]{0.49\textwidth}
        \caption{Average IPM and tokens number per texts by task.}
        \label{tab:tokens-ipm}
    \end{minipage}
}}
\end{table}

==> tables/token-ipm.tex <==
\begin{table}[H]
\begin{tabular}{l|c|c}
\toprule
 &       \textbf{IPM} &  \textbf{Num tokens} \\
 &           &             \\
\midrule
\textbf{Back Translation} & 0.88 & 12.9 \\
\textbf{Machine Translation} & 0.89 & 11.5 \\
\textbf{Zero-shot Generation} & 0.85 & 141.5 \\
\textbf{Paraphrase Generation} & 0.85 & 13.0 \\
\textbf{Simplification} & 0.86 & 18.3 \\
\textbf{Summarization} & 0.86 & 33.5  \\
\bottomrule
\end{tabular}
\caption{Average IPM and tokens number per texts by task.}
\label{tab:tokens-ipm}
\end{table}
